Mechanism to Mitigate AVX-Induced Frequency Reduction

Modern Intel CPUs reduce their frequency when executing wide vector operations (AVX2 and AVX-512 instructions), as these instructions increase power consumption. The frequency is only increased again two milliseconds after the last code section containing such instructions has been executed in order to prevent excessive numbers of frequency changes. Due to this delay, intermittent use of wide vector operations can slow down the rest of the system significantly. For example, previous work has shown the performance of web servers to be reduced by up to 10% if the SSL library uses AVX-512 vector instructions. These performance variations are hard to predict during software development as the performance impact of vectorization depends on the specific workload. We describe a mechanism to reduce the slowdown caused by wide vector instructions without requiring extensive changes to existing software. Our design allows the developer to mark problematic AVX code regions. The scheduler then restricts execution of this code to a subset of the cores so that only these cores' frequency is affected. Threads are automatically migrated to a suitable core whenever necessary. We identify a suitable load balancing policy to ensure good utilization of all available cores. Our approach is able to reduce the performance variability caused by AVX2 and AVX-512 instructions by over 70%.

==> Makefile <==
#
#  Makefile
#
#  Execute 'make help' for a list of build targets.
#

target = techreport
#paper_size ?= a4
paper_size ?= letter
pdf_quality ?= printer

all: pdf

##  Rule to generate plot output from the gnuplot input.
plot/%.eps: plot/%.plot
	@echo  "\033[35m$< --> $@\033[0m"
	gnuplot plot/term-eps-nofont.plot $< > $@

plot/%.pdf: plot/%.eps
	@echo  "\033[35m$< --> $@\033[0m"
	epstopdf $< > $@

##  Rules to generate other output
fig/%.eps: fig/%.fig
	@echo "\033[35m$< --> $@\033[0m"
	@fig2dev -L eps -p dummy $< $@

fig/%.eps: fig/%.gif
	@echo  "\033[35m$< --> $@\033[0m"
	@giftopnm $< | pnmtops -noturn -rle > $@

fig/%.eps: fig/%.prn
	@echo  "\033[35m$< --> $@\033[0m"
	@ps2eps -f $<

fig/%.eps: fig/%.ps
	@echo $(EPS)
	@echo  "\033[35m$< --> $@\033[0m"
	@ps2eps -f $<

fig/%.pdf: fig/%.eps
	@echo  "\033[35m$< --> $@\033[0m"
	epstopdf $< > $@

plotclean::
	rm -f plot/*.eps

clean::
	rm -f $(eps_targets) $(pdf_targets) *.eps rev.tex


###########################################################################
eps_targets = $(shell grep '\\epsfig\|\\includegraphics' *.tex | grep -v "\%"  | \
                    sed -e 's/file=//' | sed -e 's/,scale=.*}/}/' | \
                    sed -e 's/.*{\([^{]*\)}.*/\1.eps/;' )
$(target).dvi:: $(target).tex $(target).bib $(eps_targets)

pdf_targets = $(shell grep '\\epsfig\|\\includegraphics' *.tex | grep -v "\%"  | \
                    sed -e 's/file=//' | sed -e 's/,scale=.*}/}/' | \
                    sed -e 's/.*{\([^{]*\)}.*/\1.pdf/;' )
$(target).pdf:: $(target).tex $(target).bib $(pdf_targets)

pdf_target = $(addsuffix .pdf, $(target))
ps_target = $(addsuffix .ps, $(target))
dvi_target = $(addsuffix .dvi, $(target))

pdf: $(pdf_target)
ps: $(ps_target)
dvi: $(dvi_target)

help:
	@echo
	@echo "Automatic build target:"
	@echo "    $(pdf_target)"
	@echo "Other build target:"
	@echo "    $(ps_target)"
	@echo

clean = $(target) $(optional)

##############################################################################
#repo =  $(subst .,,$(firstword $(wildcard .git .hg)))
#
#hg_state = $(wildcard .hg/00changelog.i .hg/00changelog.d)
#git_state = $(wildcard .hg/HEAD)
#
#hg.tex: Makefile $(hg_state)
#	@changeset=`hg id | cut -f 1 -d ' '` && echo '\\renewcommand{\Revision}' "{$${changeset}}" > $@
#	-@tipdate=`hg tip | grep "date:" | cut -c 14-44` && echo '\\renewcommand{\RevisionDate}' "{$${tipdate}}" >> $@
#
#git.tex: Makefile $(git_state)
#	@changeset=`git log | head -n1 | cut -d' ' -f2` && echo '\\renewcommand{\Revision}'"{$${changeset}}" > $@
#	-@tipdate=`git log | head -n4 | grep "Date:" | cut -d' ' -f4-8` && echo '\\renewcommand{\RevisionDate}' "{$${tipdate}}" >> $@
#
#rev.tex: $(repo).tex
#	mv $< $@



timezone.tex: Makefile
	-@timezone=`date +%z` && echo '\\renewcommand{\TimeZone}' "{$${timezone}}" > $@

##############################################################################

latex = latex -interaction=batchmode $(1)
pdflatex = pdflatex $(1)
bibtex = bibtex $(1)

gs_screen = -dPDFSETTINGS=/screen
gs_printer = -dPDFSETTINGS=/printer
gs_ebook = -dPDFSETTINGS=/ebook
gs_prepress = -dPDFSETTINGS=/prepress

gs2pdf_options = -dCompatibilityLevel=1.4 $(gs_$(pdf_quality))
gs2pdf = gs -q -dSAFER -dNOPAUSE -dBATCH -sOutputFile=$(1) $(gs2pdf_options) -sDEVICE=pdfwrite -c .setpdfwrite -f $(2)

dvipdfm = dvipdfm -p $(paper_size) -o $(1) $(2)
dvips   = dvips -Pdownload35 -Pcmz -Pcmz -Pamz -t $(paper_size)  -G0 -o $(1) $(2)


RERUN = '(There were undefined references|Rerun to get (cross-references|the bars) right)'
RERUNBIB = 'No file.*\.bbl|Citation.*undefined'
UNDEFINED = '((Reference|Citation).*undefined)|(Label.*multiply defined)'
DVIPDFM_SPECIAL = 'pdf:.*docinfo'


%.pdf: %.tex $(pdf_targets)
	@echo "====> LaTeX first pass"
	$(call pdflatex,$<) || cat $*.log 
	@if egrep -q $(RERUNBIB) $*.log ; then echo "====> BibTex" && $(call bibtex,$*) && echo "====> LaTeX BibTeX pass" && $(call pdflatex, $<) ; fi
	@if egrep -q $(RERUN) $*.log ; then echo "====> LaTeX rerun" && $(call pdflatex,$<); fi; 
	@if egrep -q $(RERUN) $*.log ; then echo "====> LaTeX rerun" && $(call pdflatex,$<); fi;
	@echo "====> Undefined references and citations:"
	@egrep -i $(UNDEFINED) $*.log || echo "None."
	@echo "====> Dimensions:"
	@grep "dimension:" $*.log || echo "None."


##  Automatically choose the method to convert a DVI into a PDF, favoring
##  dvips since dvipdfm is fragile.
#%.pdf: %.dvi
#	@if egrep -q $(DVIPDFM_SPECIAL) $< ; \
#	 then echo "====> Using dvipdfm" && $(call dvipdfm,$@,$<) ; \
#	 else echo "====> Using dvips" && $(call dvips,$(<:.dvi=.ps),$<) && $(call gs2pdf,$@,$(<:.dvi=.ps)) ; \
#	 fi

##  Build a PDF from PS.  To enable, put this rule before other PDF rules.
#%.pdf: %.ps
#	@echo "====> Converting Postscript to PDF"
#	$(call gs2pdf,$@,$<)

##  Build a Postscript file from the DVI.
%.ps: %.dvi
	@echo "====> Generating Postscript"
	$(call dvips,$@,$<)

%.dvi: %.tex 
	@echo "====> LaTeX first pass"
	$(call latex,$<) || cat $*.log 
	@if egrep -q $(RERUNBIB) $*.log ; then echo "====> BibTex" && $(call bibtex,$*) && echo "====> LaTeX BibTeX pass" && $(call latex, $<) ; fi
	@if egrep -q $(RERUN) $*.log ; then echo "====> LaTeX rerun" && $(call latex,$<); fi; 
	@if egrep -q $(RERUN) $*.log ; then echo "====> LaTeX rerun" && $(call latex,$<); fi
	@echo "====> Undefined references and citations:"
	@egrep -i $(UNDEFINED) $*.log || echo "None."
	@echo "====> Dimensions:"
	@grep "dimension:" $*.log || echo "None."


clean::
	rm -rf $(addsuffix .pdf, $(clean)) $(addsuffix .ps, $(clean))
	rm -rf $(addsuffix .dvi, $(clean)) $(addsuffix .toc, $(clean))
	rm -rf $(addsuffix .log, $(clean)) $(addsuffix .aux, $(clean))
	rm -rf $(addsuffix .bbl, $(clean)) $(addsuffix .blg, $(clean))
	rm -rf $(addsuffix .out, $(clean))
	rm -rf rev.tex timezone.tex
	rm -rf $(tmp_subdirs)

##############################################################################
#  Additional dependencies
##############################################################################
rev_style = styles/ka-style.sty styles/ibm-style.sty timezone.tex

$(addsuffix .dvi, $(target) $(optional)):: $(rev_style)

##############################################################################
#
#  tex4ht - Renders html from a LaTeX file, using CSS style sheets.
#
#  To build the html output for a given LaTeX file, such as paper.tex,
#  substitute -html for .tex, such as paper-html
# 
##############################################################################

tex4ht ?= ~joshua/tex4ht.dir
tex4ht_bin = $(tex4ht)/bin/unix
tex4ht_styles = $(tex4ht)/texmf/tex/generic/tex4ht

%-html: %.tex FORCE
	mkdir -p $@
	cd $@ && env PATH=$(PATH):$(tex4ht_bin) TEXINPUTS=:..:$(tex4ht_styles) htlatex $<


==> tools/latexdiff <==
#!/usr/bin/perl -w
# latexdiff - differnces two latex files on the word level
#             and produces a latex file with the differences marked up.
#
#   Copyright (C) 2004  F J Tilmann (tilmann@esc.cam.ac.uk)
#
#    This program is free software; you can redistribute it and/or modify
#    it under the terms of the GNU General Public License Version 2 as published by
#    the Free Software Foundation.
#
#    This program is distributed in the hope that it will be useful,
#    but WITHOUT ANY WARRANTY; without even the implied warranty of
#    MERCHANTABILITY or FITNESS FOR A PARTICULAR PURPOSE.  See the
#    GNU General Public License for more details.
#
#    You should have received a copy of the GNU General Public License
#    along with this program; if not, write to the Free Software
#    Foundation, Inc., 59 Temple Place, Suite 330, Boston, MA  02111-1307  USA
#
# Detailed usage information at the end of the file
#
# Version 0.2   September 04 extension to utf-8 and variable encodings
# Version 0.1   August 04    First public release

# Inserted block for stand-alone version replaces
# use Algorithm::Diff qw(traverse_sequences);
# in standard version
# The following BEGIN block contains a verbatim copy of
# Ned Konz' Algorithm::Diff package version 1.15 except
# that all POD documentation has been stripped out.
# I encourage you to download and install the Algorithm::Diff
# package and use the standard latexdiff version instead
# (current distribution available from http://search.cpan.org/~nedkonz/Algorithm-Diff-1.15
#  the most recent version can be found via  http://search.cpan.org/search?module=Algorithm::Diff )
# Please note that the LICENCSE for Algorithm::Diff :
#   "Copyright (c) 2000-2002 Ned Konz.  All rights reserved.
#    This program is free software;
#    you can redistribute it and/or modify it under the same terms
#    as Perl itself."
# The stand-alone version of latexdiff is provided as a convenience
# for latex users with no knowledge of PERL who do not wish to install
# additional packages to be able to use latexdiff.  If you believe
# the inlining of Algorithm::Diff violates its license please contact
# me and I will modify the latexdiff distribution accordingly.
# Frederik Tilmann (tilmann@esc.cam.ac.uk)
BEGIN { 
package Algorithm::Diff;
use strict;
use vars qw($VERSION @EXPORT_OK @ISA @EXPORT);
use integer;    # see below in _replaceNextLargerWith() for mod to make
                # if you don't use this
require Exporter;
@ISA       = qw(Exporter);
@EXPORT    = qw();
@EXPORT_OK = qw(LCS diff traverse_sequences traverse_balanced sdiff);
$VERSION = sprintf('%d.%02d', (q$Revision: 1.1 $ =~ /\d+/g));

# McIlroy-Hunt diff algorithm
# Adapted from the Smalltalk code of Mario I. Wolczko, <mario@wolczko.com>
# by Ned Konz, perl@bike-nomad.com


# Create a hash that maps each element of $aCollection to the set of positions
# it occupies in $aCollection, restricted to the elements within the range of
# indexes specified by $start and $end.
# The fourth parameter is a subroutine reference that will be called to
# generate a string to use as a key.
# Additional parameters, if any, will be passed to this subroutine.
#
# my $hashRef = _withPositionsOfInInterval( \@array, $start, $end, $keyGen );

sub _withPositionsOfInInterval
{
	my $aCollection = shift;    # array ref
	my $start       = shift;
	my $end         = shift;
	my $keyGen      = shift;
	my %d;
	my $index;
	for ( $index = $start ; $index <= $end ; $index++ )
	{
		my $element = $aCollection->[$index];
		my $key = &$keyGen( $element, @_ );
		if ( exists( $d{$key} ) )
		{
			unshift ( @{ $d{$key} }, $index );
		}
		else
		{
			$d{$key} = [$index];
		}
	}
	return wantarray ? %d : \%d;
}

# Find the place at which aValue would normally be inserted into the array. If
# that place is already occupied by aValue, do nothing, and return undef. If
# the place does not exist (i.e., it is off the end of the array), add it to
# the end, otherwise replace the element at that point with aValue.
# It is assumed that the array's values are numeric.
# This is where the bulk (75%) of the time is spent in this module, so try to
# make it fast!

sub _replaceNextLargerWith
{
	my ( $array, $aValue, $high ) = @_;
	$high ||= $#$array;

	# off the end?
	if ( $high == -1 || $aValue > $array->[-1] )
	{
		push ( @$array, $aValue );
		return $high + 1;
	}

	# binary search for insertion point...
	my $low = 0;
	my $index;
	my $found;
	while ( $low <= $high )
	{
		$index = ( $high + $low ) / 2;

		#		$index = int(( $high + $low ) / 2);		# without 'use integer'
		$found = $array->[$index];

		if ( $aValue == $found )
		{
			return undef;
		}
		elsif ( $aValue > $found )
		{
			$low = $index + 1;
		}
		else
		{
			$high = $index - 1;
		}
	}

	# now insertion point is in $low.
	$array->[$low] = $aValue;    # overwrite next larger
	return $low;
}

# This method computes the longest common subsequence in $a and $b.

# Result is array or ref, whose contents is such that
# 	$a->[ $i ] == $b->[ $result[ $i ] ]
# foreach $i in ( 0 .. $#result ) if $result[ $i ] is defined.

# An additional argument may be passed; this is a hash or key generating
# function that should return a string that uniquely identifies the given
# element.  It should be the case that if the key is the same, the elements
# will compare the same. If this parameter is undef or missing, the key
# will be the element as a string.

# By default, comparisons will use "eq" and elements will be turned into keys
# using the default stringizing operator '""'.

# Additional parameters, if any, will be passed to the key generation routine.

sub _longestCommonSubsequence
{
	my $a      = shift;    # array ref
	my $b      = shift;    # array ref
	my $keyGen = shift;    # code ref
	my $compare;           # code ref

	# set up code refs
	# Note that these are optimized.
	if ( !defined($keyGen) )    # optimize for strings
	{
		$keyGen = sub { $_[0] };
		$compare = sub { my ( $a, $b ) = @_; $a eq $b };
	}
	else
	{
		$compare = sub {
			my $a = shift;
			my $b = shift;
			&$keyGen( $a, @_ ) eq &$keyGen( $b, @_ );
		};
	}

	my ( $aStart, $aFinish, $bStart, $bFinish, $matchVector ) =
	  ( 0, $#$a, 0, $#$b, [] );

	# First we prune off any common elements at the beginning
	while ( $aStart <= $aFinish
		and $bStart <= $bFinish
		and &$compare( $a->[$aStart], $b->[$bStart], @_ ) )
	{
		$matchVector->[ $aStart++ ] = $bStart++;
	}

	# now the end
	while ( $aStart <= $aFinish
		and $bStart <= $bFinish
		and &$compare( $a->[$aFinish], $b->[$bFinish], @_ ) )
	{
		$matchVector->[ $aFinish-- ] = $bFinish--;
	}

	# Now compute the equivalence classes of positions of elements
	my $bMatches =
	  _withPositionsOfInInterval( $b, $bStart, $bFinish, $keyGen, @_ );
	my $thresh = [];
	my $links  = [];

	my ( $i, $ai, $j, $k );
	for ( $i = $aStart ; $i <= $aFinish ; $i++ )
	{
		$ai = &$keyGen( $a->[$i], @_ );
		if ( exists( $bMatches->{$ai} ) )
		{
			$k = 0;
			for $j ( @{ $bMatches->{$ai} } )
			{

				# optimization: most of the time this will be true
				if ( $k and $thresh->[$k] > $j and $thresh->[ $k - 1 ] < $j )
				{
					$thresh->[$k] = $j;
				}
				else
				{
					$k = _replaceNextLargerWith( $thresh, $j, $k );
				}

				# oddly, it's faster to always test this (CPU cache?).
				if ( defined($k) )
				{
					$links->[$k] =
					  [ ( $k ? $links->[ $k - 1 ] : undef ), $i, $j ];
				}
			}
		}
	}

	if (@$thresh)
	{
		for ( my $link = $links->[$#$thresh] ; $link ; $link = $link->[0] )
		{
			$matchVector->[ $link->[1] ] = $link->[2];
		}
	}

	return wantarray ? @$matchVector : $matchVector;
}

sub traverse_sequences
{
	my $a                 = shift;                                  # array ref
	my $b                 = shift;                                  # array ref
	my $callbacks         = shift || {};
	my $keyGen            = shift;
	my $matchCallback     = $callbacks->{'MATCH'} || sub { };
	my $discardACallback  = $callbacks->{'DISCARD_A'} || sub { };
	my $finishedACallback = $callbacks->{'A_FINISHED'};
	my $discardBCallback  = $callbacks->{'DISCARD_B'} || sub { };
	my $finishedBCallback = $callbacks->{'B_FINISHED'};
	my $matchVector = _longestCommonSubsequence( $a, $b, $keyGen, @_ );

	# Process all the lines in @$matchVector
	my $lastA = $#$a;
	my $lastB = $#$b;
	my $bi    = 0;
	my $ai;

	for ( $ai = 0 ; $ai <= $#$matchVector ; $ai++ )
	{
		my $bLine = $matchVector->[$ai];
		if ( defined($bLine) )    # matched
		{
			&$discardBCallback( $ai, $bi++, @_ ) while $bi < $bLine;
			&$matchCallback( $ai,    $bi++, @_ );
		}
		else
		{
			&$discardACallback( $ai, $bi, @_ );
		}
	}

	# The last entry (if any) processed was a match.
	# $ai and $bi point just past the last matching lines in their sequences.

	while ( $ai <= $lastA or $bi <= $lastB )
	{

		# last A?
		if ( $ai == $lastA + 1 and $bi <= $lastB )
		{
			if ( defined($finishedACallback) )
			{
				&$finishedACallback( $lastA, @_ );
				$finishedACallback = undef;
			}
			else
			{
				&$discardBCallback( $ai, $bi++, @_ ) while $bi <= $lastB;
			}
		}

		# last B?
		if ( $bi == $lastB + 1 and $ai <= $lastA )
		{
			if ( defined($finishedBCallback) )
			{
				&$finishedBCallback( $lastB, @_ );
				$finishedBCallback = undef;
			}
			else
			{
				&$discardACallback( $ai++, $bi, @_ ) while $ai <= $lastA;
			}
		}

		&$discardACallback( $ai++, $bi, @_ ) if $ai <= $lastA;
		&$discardBCallback( $ai, $bi++, @_ ) if $bi <= $lastB;
	}

	return 1;
}

sub traverse_balanced
{
	my $a                 = shift;                                  # array ref
	my $b                 = shift;                                  # array ref
	my $callbacks         = shift || {};
	my $keyGen            = shift;
	my $matchCallback     = $callbacks->{'MATCH'} || sub { };
	my $discardACallback  = $callbacks->{'DISCARD_A'} || sub { };
	my $discardBCallback  = $callbacks->{'DISCARD_B'} || sub { };
	my $changeCallback    = $callbacks->{'CHANGE'};
	my $matchVector = _longestCommonSubsequence( $a, $b, $keyGen, @_ );

	# Process all the lines in match vector
	my $lastA = $#$a;
	my $lastB = $#$b;
	my $bi    = 0;
	my $ai    = 0;
	my $ma    = -1;
	my $mb;

	while (1)
	{

		# Find next match indices $ma and $mb
		do { $ma++ } while ( $ma <= $#$matchVector && !defined $matchVector->[$ma] );

		last if $ma > $#$matchVector;    # end of matchVector?
		$mb = $matchVector->[$ma];

		# Proceed with discard a/b or change events until
		# next match
		while ( $ai < $ma || $bi < $mb )
		{

			if ( $ai < $ma && $bi < $mb )
			{

				# Change
				if ( defined $changeCallback )
				{
					&$changeCallback( $ai++, $bi++, @_ );
				}
				else
				{
					&$discardACallback( $ai++, $bi, @_ );
					&$discardBCallback( $ai, $bi++, @_ );
				}
			}
			elsif ( $ai < $ma )
			{
				&$discardACallback( $ai++, $bi, @_ );
			}
			else
			{

				# $bi < $mb
				&$discardBCallback( $ai, $bi++, @_ );
			}
		}

		# Match
		&$matchCallback( $ai++, $bi++, @_ );
	}

	while ( $ai <= $lastA || $bi <= $lastB )
	{
		if ( $ai <= $lastA && $bi <= $lastB )
		{

			# Change
			if ( defined $changeCallback )
			{
				&$changeCallback( $ai++, $bi++, @_ );
			}
			else
			{
				&$discardACallback( $ai++, $bi, @_ );
				&$discardBCallback( $ai, $bi++, @_ );
			}
		}
		elsif ( $ai <= $lastA )
		{
			&$discardACallback( $ai++, $bi, @_ );
		}
		else
		{

			# $bi <= $lastB
			&$discardBCallback( $ai, $bi++, @_ );
		}
	}

	return 1;
}

sub LCS
{
	my $a = shift;                                           # array ref
	my $matchVector = _longestCommonSubsequence( $a, @_ );
	my @retval;
	my $i;
	for ( $i = 0 ; $i <= $#$matchVector ; $i++ )
	{
		if ( defined( $matchVector->[$i] ) )
		{
			push ( @retval, $a->[$i] );
		}
	}
	return wantarray ? @retval : \@retval;
}

sub diff
{
	my $a      = shift;    # array ref
	my $b      = shift;    # array ref
	my $retval = [];
	my $hunk   = [];
	my $discard = sub { push ( @$hunk, [ '-', $_[0], $a->[ $_[0] ] ] ) };
	my $add = sub { push ( @$hunk, [ '+', $_[1], $b->[ $_[1] ] ] ) };
	my $match = sub { push ( @$retval, $hunk ) if scalar(@$hunk); $hunk = [] };
	traverse_sequences( $a, $b,
		{ MATCH => $match, DISCARD_A => $discard, DISCARD_B => $add }, @_ );
	&$match();
	return wantarray ? @$retval : $retval;
}

sub sdiff
{
	my $a      = shift;    # array ref
	my $b      = shift;    # array ref
	my $retval = [];
	my $discard = sub { push ( @$retval, [ '-', $a->[ $_[0] ], "" ] ) };
	my $add = sub { push ( @$retval, [ '+', "", $b->[ $_[1] ] ] ) };
	my $change = sub {
		push ( @$retval, [ 'c', $a->[ $_[0] ], $b->[ $_[1] ] ] );
	};
	my $match = sub {
		push ( @$retval, [ 'u', $a->[ $_[0] ], $b->[ $_[1] ] ] );
	};
	traverse_balanced(
		$a,
		$b,
		{
			MATCH     => $match,
			DISCARD_A => $discard,
			DISCARD_B => $add,
			CHANGE    => $change,
		},
		@_
	);
	return wantarray ? @$retval : $retval;
}

1;
}
import Algorithm::Diff qw(traverse_sequences);
# End of inserted block for stand-alone version

use Getopt::Long ;
use strict ;
use utf8 ;

# Configuration variables: these have to be visible from the subroutines
my $MINWORDSBLOCK=3; # minimum number of tokens to form an independent block
                     # shorter identical blocks will be merged to the previous word
my $FLOATENV='(?:figure|table|plate)[\w\d*@]*' ;   # Environments in which FL variants of defined commands are used
my $PICTUREENV='(?:picture)[\w\d*@]*' ;   # Environments in which all change markup is removed

# Markup strings
# If at all possible, do not change these as parts of the program
# depend on the actual name.
# At the very least adapt subroutine postprocess to new tokens.
my $ADDMARKOPEN='\DIFaddbegin ';   # Token to mark begin of appended text
my $ADDMARKCLOSE='\DIFaddend ';   # Token to mark end of appended text
my $ADDOPEN='\DIFadd{';  # To mark begin of added text passage
my $ADDCLOSE='}';        # To mark end of added text passage
my $ADDCOMMENT='DIF > ';   # To mark added comment line
my $DELMARKOPEN='\DIFdelbegin ';   # Token to mark begin of deleted text
my $DELMARKCLOSE='\DIFdelend ';   # Token to mark end of deleted text
my $DELOPEN='\DIFdel{';  # To mark begin of deleted text passage
my $DELCLOSE='}';        # To mark end of deleted text passage
my $DELCMDOPEN='%DIFDELCMD < ';  # To mark begin of deleted commands (must begin with %, i.e., be a comment
my $DELCMDCLOSE="%%%\n";    # To mark end of deleted commands (must end with a new line)
my $DELCOMMENT='DIF < ';   # To mark deleted comment line


# main local variables:
my @TEXTCMDLIST=();  # array containing patterns of commands with text arguments
my @TEXTCMDEXCL=();  # array containing patterns of commands without text arguments (if a pattern
                     # matches bothe TEXTCMDLIST and TEXTCMDEXCL it is excluded
my @SAFECMDLIST=();  # array containing patterns of safe commands (which do not break when in the argument of DIFadd or DIFDEL)
my @SAFECMDEXCL=();

my ($i,$j,$l);
my ($old,$new);
my ($line);
my ($newpreamble,$oldpreamble);
my (@newpreamble,@oldpreamble,@diffpreamble,@diffbody);
my ($latexdiffpreamble);
my ($oldbody, $newbody, $diffbo);
my ($oldpost, $newpost);
my ($diffall);
# Option names
my ($type,$subtype,$floattype,$config,$preamblefile,$encoding,
    $showpreamble,$showsafe,$showtext,$showconfig,$showall,
    $replacesafe,$appendsafe,$excludesafe,
    $replacetext,$appendtext,$excludetext,
    $help,$verbose,$version);
my ($assign,@config);
# Defaults
$type='UNDERLINE';
$subtype='SAFE';
$floattype='FLOATSAFE';

$verbose=0;
# define character properties
sub IsNonAsciiPunct { return <<'END'    # Unicode punctuation but excluding ASCII punctuation
+utf8::IsPunct
-utf8::IsASCII
END
}
sub IsNonAsciiS { return <<'END'       # Unicode symbol but excluding ASCII
+utf8::IsS
-utf8::IsASCII
END
}


# Patterns. These are used by some of the subroutines, too
  my $pat0 = '(?:[^{}]|\\\{|\\\})*';
  my $pat1 = '(?:[^{}]|\\\{|\\\}|\{'.$pat0.'\})*';
  my $pat2 = '(?:[^{}]|\\\{|\\\}|\{'.$pat1.'\})*';
  my $pat3 = '(?:[^{}]|\\\{|\\\}|\{'.$pat2.'\})*';
  my $pat4 = '(?:[^{}]|\\\{|\\\}|\{'.$pat3.'\})*';
  my $brat0 = '(?:[^\[\]]|\\\[|\\\])*'; 

  my $quotemarks = '(?:\'\')|(?:\`\`)';
  my $punct='[0.,\/\'\`:;\"\?\(\)\[\]!~\p{IsNonAsciiPunct}\p{IsNonAsciiS}]';
  my $number='-?\d*\.\d*';
  my $mathpunct='[+=<>-^]';
  my $and = '&';
  my $coords= '[.,\s\d]*';
# word: sequence of letters or accents followed by letter
  my $word='(?:[-\w\d*]|\\\\[\"\'\`~^][A-Za-z\*])+';
  my $cmdoptseq='\\\\[\w\d\*]+(?:\['.$brat0.'\]|\{'. $pat4 . '\}|\(' . $coords .'\))*';
  my $oneletcmd='\\\\.(?:\['.$brat0.'\]|\{'. $pat4 . '\})*';
  my $math='\$(?:[^$]|\\\$)*\$';
  my $comment='%.*?\n';
  my $pat=qr/(?:\A\s*)?(?:${and}|${quotemarks}|${number}|${word}|${cmdoptseq}|${oneletcmd}|${math}|${comment}|${punct}|${mathpunct}|\{|\})\s*/ ;

  my %verbhash;

Getopt::Long::Configure('bundling');
GetOptions('type|t=s' => \$type, 
	   'subtype|s=s' => \$subtype, 
	   'floattype|f=s' => \$floattype, 
	   'config|c=s' => \$config,
	   'preamble|p=s' => \$preamblefile,
	   'encoding|e=s' => \$encoding,
	   'exclude-safecmd|A=s' => \$excludesafe,
	   'replace-safecmd=s' => \$replacesafe,
	   'append-safecmd|a=s' => \$appendsafe,
	   'exclude-textcmd|X=s' => \$excludetext,
	   'replace-textcmd=s' => \$replacetext,
	   'append-textcmd|x=s' => \$appendtext,
	   'show-preamble' => \$showpreamble,
	   'show-safecmd' => \$showsafe,
	   'show-textcmd' => \$showtext,
	   'show-config' => \$showconfig,
	   'show-all' => \$showall,
	   'verbose|V' => \$verbose,
	   'version' => \$version,
	   'help|h|H' => \$help);

if ( $help ) {
  usage() ;
}

if ( $version ) {
  die "This is LATEXDIFF 0.2 (a beta-release)\n" ;
}

if (defined($showall)){
  $showpreamble=$showsafe=$showtext=$showconfig=1;
}

# setting extra preamble commands
if (defined($preamblefile)) {
  $latexdiffpreamble=join "\n",(extrapream($preamblefile),"");
} else {
  $latexdiffpreamble=join "\n",(extrapream($type,$subtype,$floattype),"");
}

# setting up @SAFECMDLIST and @SAFECMDEXCL
if (defined($replacesafe)) {
  init_regex_arr_ext(\@SAFECMDLIST,$replacesafe);
} else {
  init_regex_arr_data(\@SAFECMDLIST, "SAFE COMMANDS");
}
if (defined($appendsafe)) {
  init_regex_arr_ext(\@SAFECMDLIST, $appendsafe);
}
if (defined($excludesafe)) {
  init_regex_arr_ext(\@SAFECMDEXCL, $excludesafe);
}

# Special: treat all cite commands as safe except in UNDERLINE mode
# (there is a conflict between citation and underline package, see
# package documentation)
if ( uc($type) ne "UNDERLINE" ) {
  push (@SAFECMDLIST, qr/^cite.*$/);
}

# setting up @TEXTCMDLIST and @TEXTCMDEXCL
if (defined($replacetext)) {
  init_regex_arr_ext(\@TEXTCMDLIST,$replacetext);
} else {
  init_regex_arr_data(\@TEXTCMDLIST, "TEXT COMMANDS");
}
if (defined($appendtext)) {
  init_regex_arr_ext(\@TEXTCMDLIST, $appendtext);
}
if (defined($excludetext)) {
  init_regex_arr_ext(\@TEXTCMDEXCL, $excludetext);
}

# setting configuration variables
if (defined($config)) {
  if (-f $config ) {
    @config=();
    open(FILE,$config) or die ("Couldn't open configuration file $config: $!");
    while (<FILE>) {
      next if /^#/ || /^%/;
      chomp;
      push (@config,$_);
    }
    close(FILE);
  }
  else {
    @config=split(",",$config);
  }
  foreach $assign ( @config ) {
    $assign=~ m/\s*(\w*)\s*=\s*(\S*)$/ or die "Illegal assignment $assign in configuration list (must be variable=value)";  
       if ( $1 eq "MINWORDSBLOCK" ) { $MINWORDSBLOCK = $2; }
       elsif ( $1 eq "FLOATENV" ) { $FLOATENV = $2 ; }
       elsif ( $1 eq "PICTUREENV" ) { $PICTUREENV = $2 ; }
       else { die "Unknown variable $1 in assignment.";}
  }
}

if ($showpreamble) {
  print "\nPreamble commands:\n";
  print $latexdiffpreamble ;
}

if ($showsafe) {
  print "\nCommands safe within scope of $ADDOPEN $ADDCLOSE and $DELOPEN $DELCLOSE (unless excluded):\n";
  print_regex_arr(@SAFECMDLIST);
  print "\nCommands not safe within scope of $ADDOPEN $ADDCLOSE and $DELOPEN $DELCLOSE :\n";
  print_regex_arr(@SAFECMDEXCL);
}
  
if ($showtext) {
  print "\nCommands with last argument textual (unless excluded):\n";
  print_regex_arr(@TEXTCMDLIST);
  print "\nCommands with last argument not textual:\n";
  print_regex_arr(@TEXTCMDEXCL);
}
    
if ($showconfig) {
  print "Configuration variables:\n";
  print "MINWORDSBLOCK=$MINWORDSBLOCK\n";
  print "FLOATENV=$FLOATENV\n";
  print "PICTUREENV=$PICTUREENV\n";
}
if ($showconfig || $showtext || $showsafe || $showpreamble) {
  exit 0; }
if ( @ARGV != 2 ) { 
  print STDERR "2 and only 2 non-option arguments required.  Write latexdiff -h to get help<n";
  exit(2);
}

# now we are done setting up and can start working   
my ($oldfile, $newfile) = @ARGV;


$encoding=guess_encoding($newfile) unless defined($encoding);

if (lc($encoding) eq "utf8" || lc($encoding) eq "ascii") {
  open (OLD, $oldfile) or die("Couldn't open $oldfile: $!");
  open (NEW, $newfile) or die("Couldn't open $newfile: $!");
  local $/ ; # locally set record operator to undefined, ie. enable whole-file mode
  $old=<OLD>;
  $new=<NEW>;
} else {
  require Encode;
  open (OLD, "<",$oldfile) or die("Couldn't open $oldfile: $!");
  open (NEW, "<",$newfile) or die("Couldn't open $newfile: $!");
  local $/ ; # locally set record operator to undefined, ie. enable whole-file mode
  $old=<OLD>;
  $new=<NEW>;
  print STDERR "Converting from $encoding to utf8\n" if $verbose;
  $old=Encode::decode($encoding,$old);
  $new=Encode::decode($encoding,$new);
}



# reset time
exetime(1);
($oldpreamble,$oldbody,$oldpost)=splitdoc($old,'\begin{document}','\end{document}');


($newpreamble,$newbody,$newpost)=splitdoc($new,'\begin{document}','\end{document}');



if ( length $oldpreamble && length $newpreamble ) {
  @oldpreamble = split /\n/, $oldpreamble;
  @newpreamble = split /\n/, $newpreamble;
  # insert dummy first line such that line count begins with line 1 (rather than perl's line 0) - just so that line numbers inserted by linediff are correct
  unshift @newpreamble,'';
  unshift @oldpreamble,'';
  print STDERR "Differencing preamble.\n" if $verbose;
  @diffpreamble = linediff(\@oldpreamble, \@newpreamble);
  # remove dummy line again
  shift @diffpreamble; 
  push @diffpreamble,$latexdiffpreamble;
  push @diffpreamble,'\begin{document}';
}
elsif ( !length $oldpreamble && !length $newpreamble ) {
  @diffpreamble=();
} else {
  print STDERR "Either both texts must have preamble or neither text must have the preamble.\n";
  exit(2);
}

print STDERR "Preprocessing body.  " if $verbose;
my ($oldleadin,$newleadin)=preprocess($oldbody,$newbody);


# run difference algorithm
@diffbody=bodydiff($oldbody, $newbody);
$diffbo=join("",@diffbody);
print STDERR "(",exetime()," s)\n","Postprocessing body. \n " if $verbose;
postprocess($diffbo);
$diffall =join("\n",@diffpreamble) ;
$diffall .= "$newleadin$diffbo" ;
$diffall .= "\\end{document}$newpost" if length $newpreamble ;
if ( lc($encoding) ne "utf8" && lc($encoding) ne "ascii" ) {
  print STDERR "Encoding output file to $encoding\n" if $verbose;
  $diffall=Encode::encode($encoding,$diffall);
  binmode STDOUT;
}
print $diffall;


print STDERR "(",exetime()," s)\n","Done.\n" if $verbose;



## guess_encoding(filename)
## reads the first 20 lines of filename and looks for call of inputenc package
## if found, return the option of this package (encoding), otherwise return ascii
sub guess_encoding {
  my ($filename)=@_;
  my ($i,$enc);
  open (FH, $filename) or die("Couldn't open $filename: $!");
  $i=0;
  while (<FH>) {
    next if /^\s*%/;    # skip comment lines
    if (m/\\usepackage\[(\w*?)\]\{inputenc\}/) {
      close(FH);
      return($1);
    }
    last if (++$i > 20 ); # scan at most 20 non-comment lines
  }
  close(FH);
  return("ascii");
}

# print_regex_arr(@arr)
# prints regex array without x-ism expansion put in by pearl to stdout
sub print_regex_arr {
  my $dumstring;
  $dumstring = join(" ",@_);     # PERL generates string (?-xism:^ref$) for quoted refex ^ref$
  $dumstring =~ s/\(\?-xism:\^(.*?)\$\)/$1/g;   # remove string and ^,$ marks before output
  print $dumstring,"\n";
}


# @lines=extrapream($type)
# reads line from appendix (end of file after __END__ token)
sub extrapream {
  my $type;
  my @retval=("%DIF PREAMBLE EXTENSION ADDED BY LATEXDIFF") ;
  my ($copy);

  while (@_) {
    $copy=0;
    $type=shift ;
    if ( -f $type ) {
      open (FILE,$type) or die "Cannot open preamble file $type: $!";
      print STDERR "Reading preamble file $type\n" if $verbose ;
      while (<FILE>) {
	chomp ;
	if ( $_ =~ m/%DIF PREAMBLE/ ) {
	  push (@retval,"$_"); 
	} else {
	  push (@retval,"$_ %DIF PREAMBLE"); 
	}
      }
    } 
    else {    # not (-f $type)
      $type=uc($type);   # upcase argument
      print STDERR "Preamble Internal Type $type\n" if $verbose;
      while (<DATA>) {
	if ( m/^%DIF $type/ ) {
	  $copy=1; }
	elsif ( m/^%DIF END $type/ ) {
	  last; }
	chomp;
	push (@retval,"$_ %DIF PREAMBLE") if $copy;
      }
      if ( $copy == 0 ) {
	print STDERR "\nPreamble style $type not implemented.\n";
        print STDERR "Write latexdiff -h to get help with available styles\n";
        exit(2);
      }
      seek DATA,0,0;    # rewind DATA handle to file begin
    }
  }
  push (@retval,"%DIF END PREAMBLE EXTENSION ADDED BY LATEXDIFF")  ;
  return @retval;
}


# ($part1,$part2,$part3)=splitdoc($text,$word1,$word2)
# splits $text into 3 parts at $word1 and $word2.
# if neither $word1 nor $word2 exist, $part1 and $part3 are empty, $part2 is $text
# If only $word1 or $word2 exist but not the other, output an error message.
sub splitdoc {
  my ($text,$word1,$word2)=@_;
  my $l1 = length $word1 ;
  my $l2 = length $word2 ;

  my $i = index($text,$word1);
  my $j = index($text,$word2);

  my ($part1,$part2,$part3)=("","","");

  if ( $i<0 && $j<0) {
    # no $word1 or $word2
    print STDERR "Old Document not a complete latex file. Assuming it is a tex file with no preamble.\n";
    $part2 = $text;
  } elsif ( $i>=0 && $j>$i ) {
    $part1 = substr($text,0,$i) ; 
    $part2 = substr($text,$i+$l1,$j-$i-$l1);
    $part3 = substr($text,$j+$l2) unless $j+$l2 >= length $text;
  } else {
    die "$word1 or $word2 not in the correct order or not present as a pair."
  }
  return ($part1,$part2,$part3);
}

# bodydiff($old,$new)
sub bodydiff {
  my ($oldwords, $newwords) = @_;
  my @retwords;

  print STDERR "(",exetime()," s)\n","Splitting into latex tokens " if $verbose;
  my @oldwords = splitlatex($oldwords);
  my @newwords = splitlatex($newwords);
  my $token;

  print STDERR "(",exetime()," s)\n","Pass 1: Expanding text commands and merging isolated identities with changed blocks  " if $verbose;
  pass1(\@oldwords, \@newwords);


  print STDERR "(",exetime()," s)\n","Pass 2: inserting DIF tokens and mark up.  " if $verbose;

  @retwords=pass2(\@oldwords, \@newwords);

  return(@retwords);
}




# @words=splitlatex($string)
# split string according to latex rules
# Each element of words is either
# a word (including trailing spaces and punctuation)
# a latex command
sub splitlatex {
  my ($string) = @_ ;
  my @retval=($string =~ m/$pat/osg);  

  if (length($string) != length(join("",@retval))) {
    print STDERR "\nWARNING: Inconsistency in length of input string and parsed string:\n";
    print STDERR "DEBUG Original length ",length($string),"  Parsed length ",length(join("",@retval)),"\n";
    print STDERR "DEBUG Input string:  |$string|\n" if (length($string)<500);
    print STDERR "DEBUG Token parsing: |",join("+",@retval),"|\n" if (length($string)<500);
    @retval=();
    # slow way only do this if other m//sg method fails
    my $last = 0;
    while ( $string =~ m/$pat/osg ) {
      my $match=$&;
      if ($last + length $& != pos $string  ) {
	my $pos=pos($string);
	my $offset=20<$last ? 20 : $last;
	my $dum=substr($string,$last-$offset,$pos-$last+$offset);
	my $dum1=$dum;
	my $cnt=$#retval;
	my $i;
	$dum1 =~ s/\n/ /g;
        print STDERR "$dum1\n";
	print STDERR " " x 20,"^" x ($pos-$last)," " x 20,"\n";
	print STDERR "Missing characters near word " . (scalar @retval) . " last: $last  pos: " .  pos($string) . " Length: " . length($match) . " Match: |$match| (indicates faulty or non-standard latex code)\n";
	# put in missing characters `by hand'
	push (@retval, substr($dum,$offset,$pos-$last-length($match)));
#       Note: there seems to be a bug in substr with utf8 that made the following line output substr which were too long,
#             using dum instead appears to work
#	push (@retval, substr($string,$last, pos($string)-$last-length($match)));
      }
      push (@retval, $match);
      $last=pos $string;
    }

  }
  return @retval;
}


# pass1( \@seq1,\@seq2)
# Look for differences between seq1 and seq2.
# Where an common-subsequence block is flanked by deleted or appended blocks, 
# and is shorter than $MINWORDSBLOCK words it is appended
# to the last deleted or appended word.  If the block contains tokens other than words 
# or punctuation it is not merged.
# Deleted or appended block consisting of words and safe commands only are
# also merged, to prevent break-up in pass2 (after previous isolated words have been removed)
# If there are commands with textual arguments (e.g. \caption) both in corresponding 
# appended and deleted blocks split them such that the command and opening bracket 
# are one token, then the rest is split up following standard rules, and the closing 
# bracket is a separate token, ie. turn
# "\caption{This is a textual argument}" into 
# ("\caption{","This ","is ","a ","textual ","argument","}")
# No return value.  Destructively changes sequences
sub pass1 {
  my $seq1 = shift ;
  my $seq2 = shift ;

  my $len1 = scalar @$seq1;
  my $len2 = scalar @$seq2;
  my $wpat=qr/^(?:[a-zA-Z.,'`:;?()!]*)[\s~]*$/;   #'

  my ($last1,$last2)=(-1,-1) ;
  my $cnt=0;
  my $block=[];
  my $addblock=[];
  my $delblock=[];
  my $todo=[];
  my $instruction=[];
  my $i;
  my (@delmid,@addmid,@dummy);

  my ($addcmds,$delcmds,$matchindex);
  my ($addtextblocks,$deltextblocks);
  my ($addtokcnt,$deltokcnt,$mattokcnt)=(0,0,0);
  my ($addblkcnt,$delblkcnt,$matblkcnt)=(0,0,0);

  my $adddiscard = sub {
                      if ($cnt > 0 ) {
			$matblkcnt++;
			# just after an unchanged block 
#			print STDERR "Unchanged block $cnt, $last1,$last2 \n";
                        if ($cnt < $MINWORDSBLOCK 
			    && $cnt==scalar (
				     grep { /^$wpat/ || ( /^\\([\w\d\*]+)((?:\[$brat0\]|\{$pat4\})*)/o 
							   && iscmd($1,\@SAFECMDLIST,\@SAFECMDEXCL) 
							   && scalar(@dummy=split(" ",$2))<3 ) }
					     @$block) )  {
			  # merge identical blocks shorter than $MINWORDSBLOCK 
			  # and only containing ordinary words
			  # with preceding different word
			  # We cannot carry out this merging immediately as this
			  # would change the index numbers of seq1 and seq2 and confuse
			  # the algorithm, instead we store in @$todo where we have to merge
                          push(@$todo, [ $last1,$last2,$cnt,@$block ]);
			}
			$block = []; 
			$cnt=0; $last1=-1; $last2=-1;
		      }
		    };
  my $discard=sub { $deltokcnt++;
                    &$adddiscard; #($_[0],$_[1]);
		    push(@$delblock,[ $seq1->[$_[0]],$_[0] ]);
		    $last1=$_[0] };		      

  my $add =   sub { $addtokcnt++;
                    &$adddiscard; #($_[0],$_[1]);
		    push(@$addblock,[ $seq2->[$_[1]],$_[1] ]);
		    $last2=$_[1] };		      

  my $match = sub { $mattokcnt++;
                    if ($cnt==0) {   # first word of matching sequence after changed sequence or at beginning of word sequence
		      $deltextblocks = extracttextblocks($delblock); 
		      $delblkcnt++ if scalar @$delblock;
		      $addtextblocks = extracttextblocks($addblock);
		      $addblkcnt++ if scalar @$addblock;

		      $delcmds = extractcommands($delblock);
      		      $addcmds = extractcommands($addblock);
		      # keygen(third argument of _longestCommonSubsequence) implies to sort on command (0th elements of $addcmd elements)
		      $matchindex=Algorithm::Diff::_longestCommonSubsequence($delcmds,$addcmds, sub { $_[0]->[0] } );
		      
		      for ($i=0 ; $i<=$#$matchindex ; $i++) {
			if (defined($matchindex->[$i])){
			  $j=$matchindex->[$i];
			  @delmid=splitlatex($delcmds->[$i][3]);
			  @addmid=splitlatex($addcmds->[$j][3]);

			  while (scalar(@$deltextblocks) && $deltextblocks->[0][0]<$delcmds->[$i][2]) {
			    my ($index,$block,$cnt)=@{ shift(@$deltextblocks) };
			    push(@$todo, [$index,-1,$cnt,@$block]);
			  }
			  push(@$todo, [ $delcmds->[$i][1],-1,-1,$delcmds->[$i][2],@delmid,$delcmds->[$i][4]]);

			  while (scalar(@$addtextblocks) && $addtextblocks->[0][0]<$addcmds->[$j][2]) {
			    my ($index,$block,$cnt)=@{ shift(@$addtextblocks) };
			    push(@$todo, [-1,$index,$cnt,@$block]);
			  }
			  push(@$todo, [ -1,$addcmds->[$j][1],-1,$addcmds->[$j][2],@addmid,$addcmds->[$j][4]]);
			}
		      }
		      # mop up remaining textblocks
		      while (scalar(@$deltextblocks)) {
			my ($index,$block,$cnt)=@{ shift(@$deltextblocks) } ;
			push(@$todo, [$index,-1,$cnt,@$block]);
		      }
		      while (scalar(@$addtextblocks)) {
			my ($index,$block,$cnt)=@{ shift(@$addtextblocks) };
			push(@$todo, [-1,$index,$cnt,@$block]);
		      }
		      
		      $addblock=[];
		      $delblock=[];
		    }
		    push(@$block,$seq2->[$_[1]]);  
		    $cnt++  };

  my $keyfunc = sub { join("  ",split(" ",shift())) };

  traverse_sequences($seq1,$seq2, { MATCH=>$match, DISCARD_A=>$discard, DISCARD_B=>$add }, $keyfunc );


  # now carry out the merging/splitting.  Refer to elements relative from 
  # the end (with negative indices) as these offsets don't change before the instruction is executed
  # cnt>0: merged small unchanged groups with previous changed blocks
  # cnt==-1: split textual commands into components
  foreach $instruction ( @$todo) {
    ($last1,$last2,$cnt,@$block)=@$instruction ;
    if ($cnt>=0) {
      splice(@$seq1,$last1-$len1,1+$cnt,join("",$seq1->[$last1-$len1],@$block)) if $last1>=0;
      splice(@$seq2,$last2-$len2,1+$cnt,join("",$seq2->[$last2-$len2],@$block)) if $last2>=0;
    } else {
      splice(@$seq1,$last1-$len1,1,@$block) if $last1>=0;
      splice(@$seq2,$last2-$len2,1,@$block) if $last2>=0;
    }
  }

  if ($verbose) { 
    print STDERR "\n";
    print STDERR "  $mattokcnt matching  tokens in $matblkcnt blocks.\n";
    print STDERR "  $deltokcnt discarded tokens in $delblkcnt blocks.\n";
    print STDERR "  $addtokcnt appended  tokens in $addblkcnt blocks.\n";
  }
}


# extracttextblocks(\@blockindex)
# $blockindex has the following format 
# [ [ token1, index1 ], [token2, index2],.. ] 
# where index refers to the index in the original old or new word sequence 
# Returns: reference to an array of the form  
# [[ $index, $textblock, $cnt ], ..
# where $index index of block to be merged
#       $textblock contains all the words to be merged with the word at $index (but does not contain this word)
#       $cnt   is length of block
#
# requires: iscmd
#
sub extracttextblocks { 
  my $block=shift;
  my ($i,$token,$index);
  my $textblock=[];
  my $last=-1;
  my $wpat=qr/^(?:[a-zA-Z.,'`:;?()!]*)[\s~]*$/;  #'
  my $retval=[];
		 
  for ($i=0;$i< scalar @$block;$i++) {
    ($token,$index)=@{ $block->[$i] };

    # store pure text blocks
    if ($token =~ /$wpat/ ||  ( $token =~/^\\([\w\d\*]+)((?:\[$brat0\]|\{$pat4\})*)/o 
				&& iscmd($1,\@SAFECMDLIST,\@SAFECMDEXCL) 
				&& !iscmd($1,\@TEXTCMDLIST,\@TEXTCMDEXCL))) {
      # we have text or a command which can be treated as text
      if ($last<0) {
	# new pure-text block
	$last=$index;
      } else {
	# add to pure-text block
	push(@$textblock, $token); 
      }
    } else {
      # it is not text
      if (scalar(@$textblock)) {
	push(@$retval,[ $last, $textblock, scalar(@$textblock) ]);
      }
      $textblock=[];
      $last=-1;
    }
  }
  # finish processing a possibly unfinished block before returning
  if (scalar(@$textblock)) {
    push(@$retval,[ $last, $textblock, scalar(@$textblock) ]);
  }
  return($retval)
}



# extractcommands( \@blockindex )
# $blockindex has the following format 
# [ [ token1, index1 ], [token2, index2],.. ] 
# where index refers to the index in the original old or new word sequence 
# Returns: reference to an array of the form  
# [ [ "\cmd1", "\cmd1[optarg]{arg1}{", "arg2" ,"} ",index ],.. 
# where index is just taken from input array 
# command must have a textual argument as last argument 
# 
# requires: iscmd 
# 
sub extractcommands { 
  my $block=shift;
  my ($i,$token,$index,$cmd,$open,$mid,$closing);
  my $retval=[];

  for ($i=0;$i< scalar @$block;$i++) {
    ($token,$index)=@{ $block->[$i] };
    # check if token is an alphanumeric command sequence with at least one non-optional argument
    # \cmd[...]{...}{last argument}  
    # Capturing in the following results in these associations
    # $1: \cmd[...]{...}{
    # $2: \cmd
    # $3: last argument
    # $4: }  + trailing spaces
    if ( ( $token =~ m/^(\\([\w\d\*]+)(?:\[$brat0\]|\{$pat4\})*\{)($pat4)(\}\s*)$/so )
	 && iscmd($2,\@TEXTCMDLIST,\@TEXTCMDEXCL) ) {
      #      push(@$retval,[ $2,$index,$1,$3,$4 ]);
      ($cmd,$open,$mid,$closing) = ($2,$1,$3,$4) ;
      $closing =~ s/\}/\\RIGHTBRACE/ ;
      push(@$retval,[ $cmd,$index,$open,$mid,$closing ]);
    }
  }
  return $retval;
}

# iscmd($cmd,\@regexarray,\@regexexcl) checks
# return 1 if $cmd matches any of the patterns in the 
# array $@regexarray, and none of the patterns in \@regexexcl, otherwise return 0
sub iscmd {
  my ($cmd,$regexar,$regexexcl)=@_;
  my ($ret)=0;
  foreach $pat ( @$regexar ) {
    if ( $cmd =~ m/^${pat}$/ ) {
      $ret=1 ; 
      last;
    }
  }
  return 0 unless $ret;
  foreach $pat ( @$regexexcl ) {
    return 0 if ( $cmd =~ m/^${pat}$/ );
  }
  return 1;
}


# pass2( \@seq1,\@seq2)
# Look for differences between seq1 and seq2.  
# Mark begin and end of deleted and appended sequences with tags $DELOPEN and $DELCLOSE
# and $ADDOPEN and $ADDCLOSE, respectively, however exlclude { } & and all comands, unless
# they match an element of the whitelist
# Deleted comment lines are marked with %DIF < 
# Added comment lines are marked with %DIF > 
sub pass2 {
  my $seq1 = shift ;
  my $seq2 = shift ;

  my ($addtokcnt,$deltokcnt,$mattokcnt)=(0,0,0);
  my ($addblkcnt,$delblkcnt,$matblkcnt)=(0,0,0);

  my $retval = [];
  my $delhunk   = [];
  my $addhunk   = [];

  my $discard = sub { $deltokcnt++;
                      push ( @$delhunk, $seq1->[$_[0]]) };

  my $add = sub { $addtokcnt++;
                  push ( @$addhunk, $seq2->[$_[1]]) };

  my $match = sub { $mattokcnt++;
                    if ( scalar @$addhunk ) {
                      $addblkcnt++;
                      # we mark up changes, but simply quote commands
                      push @$retval,marktags($ADDMARKOPEN,$ADDMARKCLOSE,$ADDOPEN,$ADDCLOSE,"","",$ADDCOMMENT,$addhunk);
		      $addhunk = [];
		    }
		    if ( scalar @$delhunk ) {
                      $delblkcnt++;
		      # mark up changes, but comment out commands
                      push @$retval,marktags($DELMARKOPEN,$DELMARKCLOSE,$DELOPEN,$DELCLOSE,$DELCMDOPEN,$DELCMDCLOSE,$DELCOMMENT,$delhunk);
		      $delhunk = [];
		    }
		    push(@$retval,$seq2->[$_[1]]) };
 
  my $keyfunc = sub { join("  ",split(" ",shift())) };

  traverse_sequences($seq1,$seq2, { MATCH=>$match, DISCARD_A=>$discard, DISCARD_B=>$add }, $keyfunc );
  # clear up unprocessed hunks
  push @$retval,marktags($ADDMARKOPEN,$ADDMARKCLOSE,$ADDOPEN,$ADDCLOSE,"","",$ADDCOMMENT,$addhunk) if scalar @$addhunk;
  push @$retval,marktags($DELMARKOPEN,$DELMARKCLOSE,$DELOPEN,$DELCLOSE,$DELCMDOPEN,$DELCMDCLOSE,$DELCOMMENT,$delhunk) if scalar @$delhunk;

  if ($verbose) { 
    print STDERR "\n";
    print STDERR "  $mattokcnt matching  tokens. \n";
    print STDERR "  $deltokcnt discarded tokens in $delblkcnt blocks.\n";
    print STDERR "  $addtokcnt appended  tokens in $addblkcnt blocks.\n";
  }

  return(@$retval);
}

# marktags($openmark,$closemark,$open,$close,$opencmd,$closecmd,$comment,\@block)
# returns ($openmark,$open,$block,$close,$closemark) if @block only contains no commands (except white-listed ones),
# braces, ampersands, or comments
# mark comments with $comment
# exclude all other exceptions from scope of open, close like this
# ($openmark, $open,...,$close, $opencomd,command, command,$closecmd, $open, ..., $close, $closemark)
sub marktags {
  my ($openmark,$closemark,$open,$close,$opencmd,$closecmd,$comment,$block)=@_;
  my $word;
  my $retval=[];
  my $noncomment=0;
  my $cmd=-1;    # -1 at beginning 0: last token written is a ordinary word 1: last token written is a command
                # for keeping track whether we are just in a command sequence or in a word sequence
  my $cmdcomment= ($opencmd =~ m/^%/);  # Flag to indicate whether opencmd is a comment (i.e. if we intend to simply comment out changed commands)

# split this block to flatten out sequences joined in pass1
  @$block=splitlatex(join "",@$block);
  foreach (@$block) {
    $word=$_; 
    if ( $word =~ s/^%/%$comment/ ) {
      push (@$retval,$word); 
      next;
    }
    if (! $noncomment) {
      push (@$retval,$openmark); 
      $noncomment=1;
    }
    if ( $word =~ /^[&{}\[\]]/ || ( $word =~ /^\\([\w*@]*)/ && !iscmd($1,\@SAFECMDLIST,\@SAFECMDEXCL)) ) {
      # word is a command or other significant token
      push (@$retval,$opencmd) if $cmd==-1 ;
      push (@$retval,$close,$opencmd) if $cmd==0 ;
      $word =~ s/\n/\n${opencmd}/sg if $cmdcomment ;   # if opencmd is a comment, repeat this at the beginning of every line
      push (@$retval,$word);
      $cmd=1;
    } else {
      push (@$retval,$open) if $cmd==-1 ;
      push (@$retval,$closecmd,$open) if $cmd==1 ;
      push (@$retval,$word);
      $cmd=0;
    }
  }
  push (@$retval,$close) if $cmd==0;
  push (@$retval,$closecmd) if $cmd==1;

  push (@$retval,$closemark) if ($noncomment);
  return @$retval;
}

# preprocess($string, ..)
# carry out the following pre-processing steps for all arguments:
# 1. Remove leading white-space
# 2. mark all first empty line (in block of several) with \PAR tokens
# 3. Convert all '\%' into '\PERCENTAGE ' to make parsing regular expressions easier
# 4. Convert all \verb|some verbatim text| commands (where | can be an arbitrary character)
#    into \verb{hash}
# 5. Convert \begin{verbatim} some verbatim text \end{verbatim} into \verbatim{hash}
sub preprocess {
  my @leadin=() ;
  for (@_) { 
    s/^(\s*)//s;
    push(@leadin,$1);
    s/\n(\s*?)\n((?:\s*\n)*)/\n$1\\PAR\n$2/g ;
    s/(?<!\\)\\%/\\PERCENTAGE /g ;  # (?<! is negative lookbehind assertion to prevent \\% from being converted
    s/(\\verb\*?)(\S)(.*?)\2/"${1}{". tohash(\%verbhash,"${2}${3}${2}") ."}"/esg;
    s/\\begin\{(verbatim\*?)\}(.*?)\\end\{\1\}/"\\${1}{". tohash(\%verbhash,"${2}") . "}"/esg;
  }
  return(@leadin);
}

#hashstring=tohash(\%hash,$string)
# creates a hash value based on string and stores in %hash
sub tohash {
  my ($hash,$string)=@_;
  my (@arr,$val);
  my ($sum,$i)=(0,1);
  my ($hstr);

  @arr=unpack('c*',$string);

  foreach $val (@arr) {
    $sum += $i*$val;
    $i++;
  }
  $hstr= "$sum";
  if (defined($hash->{$hstr}) && $string ne $hash->{$hstr}) {
    warn "Repeated hash value for verbatim mode in spite of different content.";
    $hstr="-$hstr";
  }
  $hash->{$hstr}=$string;
  return($hstr);
}

#string=fromhash(\%hash,$fromstring)
# restores string value stored in hash
#string=fromhash(\%hash,$fromstring,$prependstring)
# additionally begins each line with prependstring
sub fromhash {
  my ($hash,$hstr)=($_[0],$_[1]);
  my $retstr=$hash->{$hstr};
  if ( $#_ >= 2) {
    $retstr =~ s/^/$_[2]/mg;
  }
  return $retstr;
}


# postrocess($string, ..)
# carry out the following post-processing steps for all arguments:
# Replace \RIGHTBRACE by }
# Convert DIFadd, DIFdel, DIFFaddbegin , ... into FL varieties
#    within floats (currently recognised float environments: plate,table,figure
#    plus starred varieties).
# Remove DIFadd, DIFdel, DIFFaddbegin , ... from picture environments
# 1. Remove empty %DIFCMD < lines 
# 2. Expand hashes of verb and verbatim environments
# 3. Convert '\PERCENTAGE ' back into '\%'
# 4. remove all \PAR tokens
#
# Note have to manually synchronize substitution commands below and 
# DIF.. command names in the header
sub postprocess {
  my ($begin,$len,$cnt,$float);

  for (@_) { 
    # Replace \RIGHTBRACE by }    
    s/\\RIGHTBRACE/}/g;
    # change begin and end commands within comments such that they don't disturb the pattern matching (if there are several \begin or \end in one line
    # this substitution is insufficient but that appears unlikely
    s/(%.*)\\begin\{(.*)$/$1\\BEGINDIF\{$2/mg ;
    s/(%.*)\\end\{(.*)$/$1\\ENDDIF\{$2/mg ;
    # Convert DIFadd, DIFdel, DIFFaddbegin , ... into  varieties
    #    within floats (currently recognised float environments: plate,table,figure
    #    plus starred varieties.
    while ( m/\\begin\{($FLOATENV)\}.*?\\end\{\1\}/sg ) {
      $cnt=0;
      $len=length($&);
      $begin=pos($_) - $len;
      $float=$&;
      $float =~ s/\\DIFaddbegin /\\DIFaddbeginFL /g;
      $float =~ s/\\DIFaddend /\\DIFaddendFL /g;
      $float =~ s/\\DIFadd\{/\\DIFaddFL{/g;
      $float =~ s/\\DIFdelbegin /\\DIFdelbeginFL /g;
      $float =~ s/\\DIFdelend /\\DIFdelendFL /g;
      $float =~ s/\\DIFdel\{/\\DIFdelFL{/g;
      substr($_,$begin,$len)=$float;
      pos = $begin + length($float);
    }
    # Remove all mark up within picture environments
    while ( m/\\begin\{($PICTUREENV)\}.*?\\end\{\1\}/sg ) {
      $cnt=0;
      $len=length($&);
      $begin=pos($_) - $len;
      $float=$&;
      $float =~ s/\\DIFaddbegin //g;
      $float =~ s/\\DIFaddend //g;
      $float =~ s/\\DIFadd\{($pat4)\}/$1/g;
      $float =~ s/\\DIFdelbegin //g;
      $float =~ s/\\DIFdelend //g;
      $float =~ s/\\DIFdel\{($pat4)\}//g;
      substr($_,$begin,$len)=$float;
      pos = $begin + length($float);
    }
    # undo renaming of the \begin and \end in comments
    s/(%.*)\\BEGINDIF\{(.*)$/$1\\begin\{$2/mg ;
    s/(%.*)\\ENDDIF\{(.*)$/$1\\end\{$2/mg ;
    # remove empty DIFCMD < lines
    s/^\Q${DELCMDOPEN}\E\n//msg;
    # Expand hashes of verb and verbatim environments (note negative look behind assertion to not leak out of DIFCMD comments
    s/(\\verb\*?)\{([-\d]*?)\}/"${1}". fromhash(\%verbhash,$2)/esg;
    s/${DELCMDOPEN}\\(verbatim\*?)\{([-\d]*?)\}/"${DELCMDOPEN}\\begin{${1}}".fromhash(\%verbhash,$2,$DELCMDOPEN)."${DELCMDOPEN}\\end{${1}}"/esg;
    s/\\(verbatim\*?)\{([-\d]*?)\}/"\\begin{${1}}".fromhash(\%verbhash,$2)."\\end{${1}}"/esg;
    # Convert '\PERCENTAGE ' back into '\%'			       
    s/\\PERCENTAGE /\\%/g;
    # remove all \PAR tokens (taking care to properly keep commented out PAR's
    # from introducing uncommented newlines - next line)
    s/(%DIF < )([^\n]*?)\\PAR\n/$1$2\n$1\n/sg;
    s/\\PAR\n/\n/sg;
    }

  return;
}


# @diffs=linediff(\@seq1, \@seq2)
# mark up lines like this
#%DIF mm-mmdnn
#%< old deleted line(s)
#%DIF -------
#%DIF mmann-nn
#new appended line %< 
#%DIF -------
# Future extension: mark change explicitly
# Assumes: traverse_sequence traverses deletions before insertions in changed sequences
#          all line numbers relative to line 0 (first line of real file)
sub linediff {
  my $seq1 = shift ;
  my $seq2 = shift ;

  my $block = [];
  my $retseq = [];
  my @begin=('','',''); # dummy initialisation
  my $instring ; 

  my $discard = sub { @begin=('d',$_[0],$_[1]) unless scalar @$block ; 
                      push(@$block, "%DIF < " . $seq1->[$_[0]]) };
  my $add = sub { if (! scalar  @$block) {
		    @begin=('a',$_[0],$_[1]) ;}
		  elsif ( $begin[0] eq 'd' ) {
                    $begin[0]='c'; $begin[2]=$_[1];
		    push(@$block, "%DIF -------") }
                  push(@$block,  $seq2->[$_[1]] . " %DIF > " ) };
  my $match = sub { if ( scalar @$block ) {
                      if ( $begin[0] eq 'd' && $begin[1]!=$_[0]-1) {
			$instring = sprintf "%%DIF %d-%dd%d",$begin[1],$_[0]-1,$begin[2]; }
		      elsif ( $begin[0] eq 'a' && $begin[2]!=$_[1]-1) {
			$instring = sprintf "%%DIF %da%d-%d",$begin[1],$begin[2],$_[1]-1; }
		      elsif ( $begin[0] eq 'c' ) {
			$instring = sprintf "%%DIF %sc%s",
			                     ($begin[1]==$_[0]-1) ? "$begin[1]" : $begin[1]."-".($_[0]-1)  , 
			                     ($begin[2]==$_[1]-1) ? "$begin[2]" : $begin[2]."-".($_[1]-1)  ; }
		      else {
			$instring = sprintf "%%DIF %d%s%d",$begin[1],$begin[0],$begin[2]; }
		      push @$retseq, $instring,@$block, "%DIF -------" ; 
		      $block = []; 
		    }
		    push @$retseq, $seq2->[$_[1]]
		  };
  # key function: remove multiple spaces (such that insertion or deletion of redundant white space is not reported)
  my $keyfunc = sub { join("  ",split(" ",shift())) };

  traverse_sequences($seq1,$seq2, { MATCH=>$match, DISCARD_A=>$discard, DISCARD_B=>$add }, $keyfunc );
  push @$retseq, @$block if scalar @$block; 

  return wantarray ? @$retseq : $retseq ;
}



# init_regex_arr_data(\@array,"TOKEN INIT")
# scans DATA file handel for line "%% TOKEN INIT" line
# then appends each line not beginning with % into array (as a quoted regex)
sub init_regex_arr_data {
  my ($arr,$token)=@_;
  my ($copy);
  while (<DATA>) {
    if ( m/^%%BEGIN $token\s*$/ ) {
      $copy=1; }
    elsif ( m/^%%END $token\s*/ )  {
      last; }
    chomp;
    push (@$arr,qr/^$_$/) if ( $copy && !/^%/ ) ;
  }
  seek DATA,0,0;    # rewind DATA handle to file begin
}


# init_regex_arr_ext(\@array,$arg)
# fills array with regular expressions.
# if arg is a file name, then read in list of regular expressions from that file
# (one expression per line)
# Otherwise treat arg as a comma separated list of regular expressions
sub init_regex_arr_ext {
  my ($arr,$arg)=@_;
  my $regex;
  if ( -f $ arg ) {
    open(FILE,"$arg") or die ("Couldn't open $arg: $!");
    while (<FILE>) {
      next if /^#/ || /^%/;
      chomp;
      push (@$arr,qr/^$_$/);
    }
    close(FILE);
  }
  else {
    # assume it is a comma-separated list of reg-ex
    foreach $regex (split(qr/(?<!\\),/,$arg)) {
      $regex =~ s/\\,/,/g;
      push (@$arr,qr/^$regex$/);
    }
  }
}

#exetime() returns time since last execution of this command
#exetime(1) resets this time
my $lasttime=-1;   # global variable for persistence
sub exetime {
  my $reset=0;
  my $retval;
  if ((scalar @_) >=1) {
    $reset=shift;
  }
  if ($reset) {
    $lasttime=times();
  }
  else {
    $retval=times()-$lasttime;
    $lasttime=$lasttime+$retval;
    return($retval);
  }
}


sub usage {
  die <<"EOF"; 
Usage: $0 [options] old.tex new.tex > diff.tex

Compares two latex files and writes tex code to stdout, which has the same
format as new.tex but has all changes relative to old.tex marked up or commented.

--type=markupstyle
-t markupstyle         Add code to preamble for selected markup style
                       Available styles: UNDERLINE CTRADITIONAL TRADITIONAL CFONT INVISIBLE 
                                         CHANGEBAR CCHANGEBAR CULINECHBAR CFONTCBHBAR
                       [ Default: UNDERLINE ]

--subtype=markstyle
-s markstyle           Add code to preamble for selected style for bracketing
                       commands (e.g. to mark changes in  margin)
                       Available styles: SAFE MARGINAL DVIPSCOL
                       [ Default: SAFE ]

--floattype=markstyle
-f markstyle           Add code to preamble for selected style which 
                       replace standard marking and markup commands within floats
                       (e.g., marginal remarks cause an error within floats
                       so marginal marking can be disabled thus)
                       Available styles: FLOATSAFE IDENTICAL
                       [ Default: FLOATSAFE ]

--encoding=enc
-e enc                 Specify encoding of old.tex and new.tex. Typical encodings are
                       ascii, utf8, latin1, latin9.  A list of available encodings can be 
                       obtained by executing 
                       perl -MEncode -e 'print join ("\n",Encode->encodings( ":all" )) ;'
                       [Default encoding is utf8 unless the first few lines of the preamble contain
                       an invocation "\\usepackage[..]{inputenc} in which case the 
                       encoding chosen by this command is asssumed. Note that ASCII (standard
                       latex) is a subset of utf8]

--preamble=file
-p file                Insert file at end of preamble instead of auto-generating
                       preamble.  The preamble must define the following commands
                       \\DIFaddbegin,\\DIFaddend,\\DIFadd{..},
                       \\DIFdelbegin,\\DIFdelend,\\DIFdel{..},
                       and varieties for use within floats
                       \\DIFaddbeginFL,\\DIFaddendFL,\\DIFaddFL{..},
                       \\DIFdelbeginFL,\\DIFdelendFL,\\DIFdelFL{..}
                       (If this option is set -t, -s, and -f options
                       are ignored.)

--exclude-safecmd=exclude-file
--exclude-safecmd="cmd1,cmd2,..."
-A exclude-file 
--replace-safecmd=replace-file
--append-safecmd=append-file
--append-safecmd="cmd1,cmd2,..."
-a append-file         Exclude from, replace or append to the list of regex
                       matching commands which are safe to use within the 
                       scope of a \\DIFadd or \\DIFdel command.  The file must contain
                       one Perl-RegEx per line (Comment lines beginning with # or % are
                       ignored). A literal comma within the comma-separated list must be
                       escaped thus "\\,",   Note that the RegEx needs to match the whole of 
                       the token, i.e., /^regex\$/ is implied and that the initial
                       "\\" of the command is not included. The --exclude-safecmd
                       option can be combined with either of the other two.

--exclude-textcmd=exclude-file 
--exclude-textcmd="cmd1,cmd2,..."
-X exclude-file
--replace-textcmd=replace-file
--append-textcmd=append-file
--append-textcmd="cmd1,cmd2,..."
-x append-file         Exclude from, replace or append to the list of regex
                       matching commands whose last argument is text.  See
                       entry for --exclude-safecmd directly above for further details.

--config var1=val1,var2=val2,...
-c var1=val1,..        Set configuration variables.
-c configfile           Available variables: 
                          MINWORDSBLOCK (integer)
                          FLOATENV (RegEx)
                          PICTUREENV (RegEx)

--show-preamble        Print generated or included preamble commands to stdout.

--show-safecmd         Print list of regex matching and excluding safe commands.

--show-textcmd         Print list of regex matching and excluding commands with text argument.

--show-config          Show values of configuration variables

   NB For all --show commands, no old.tex or new.tex file needs to be given, and no 
      differencing takes place.

--verbose
-V                     Output various status information to stderr during processing.
                       Default is to work silently.

--help
-h                     Show this help text.

--version              Show version number.
EOF
}

=head1 NAME

latexdiff - determine and markup differences between two latex files

=head1 SYNOPSIS

B<latexdiff> [ B<OPTIONS> ] F<old.tex> F<new.tex> > F<diff.tex>

=head1 DESCRIPTION

Briefly, I<latexdiff> is a utility program to aid in the management of
revisions of latex documents. It compares two valid latex files, here
called C<old.tex> and C<new.tex>, finds significant differences
between them (i.e., ignoring the number of white spaces and position
of line breaks), and adds special commands to highlight the
differences.  Where visual highlighting is not possible, e.g. for changes
in the formatting, the differences are
nevertheless marked up in the source.

The program treats the preamble differently from the main document.
Differences between the preambles are found using line-based
differencing (similarly to the Unix diff command, but ignoring white
spaces).  A comments, "C<%DIF E<gt>>" is appended to each added line, i.e. a 
line present in C<new.tex> but not in C<old.tex>.  Discarded lines 
 are deactivated by prepending "C<%DIF E<lt>>". Changed blocks are preceded  by
comment lines giving information about line numbers in the original files.  Where there are insignificant
differences, the resulting file C<diff.tex> will be similar to
C<new.tex>.  At the end of the preamble, the definitions for I<latexdiff> markup commands are inserted.
In differencing the main body of the text, I<latexdiff> attempts to
satisfy the following guidelines (in order of priority):

=over 3

=item 1

If both C<old.tex> and C<new.tex> are valid LaTeX, then the resulting
C<diff.tex> should also be valid LateX. (NB If a few plain TeX commands
are used within C<old.tex> or C<new.tex> then C<diff.tex> is not
guaranteed to work but usually will).

=item 2

Significant differences are determined on the level of
individual words. All significant differences, including differences
between comments should be clearly marked in the resulting source code
C<diff.tex>.

=item 3

If a changed passage contains text or text-producing commands, then
running C<diff.tex> through LateX should produce output where added
and discarded passages are highlighted.

=item 4

Where there are insignificant differences, e.g. in the positioning of
line breaks, C<diff.tex> should follow the formatting of C<new.tex>

=back

For differencing the same algorithm as I<diff> is used but words
instead of lines words are compared.  An attempt is made to recognize
blocks which are completely changed such that they can be marked up as unit
(otherwise readibility is reduced because common words such as "the" and "and" which can be found both in the discarded and added block are considered to be identical text parts and thus not marked up, and added and discarded
text parts are interspersed between these common words).
Comments are differenced line by line
but the number of spaces within comments is ignored. Commands including
all their arguments are generally compared as one unit, i.e., no mark-up
is inserted into the arguments of commands.  However, for a selected
number of commands (for example, C<\caption> and all sectioning
commands) the last argument is known to be text. This text is
split into words and differenced just as ordinary text (use options to
show and change the list of text commands, see below). As the
algorithm has no detailed knowledge of LaTeX, it assumes all pairs of
curly braces immediately following a command (i.e. a sequence of
letters beginning with a backslash) are arguments for that command.
As a restriction to condition 1 above it is thus necessary to surround
all arguments with curly braces, and to not insert
extraneous spaces.  For example, write 

  \section{\textem{This is an emphasized section title}}

and not

  \section {\textem{This is an emphasized section title}}

or

  \section\textem{This is an emphasized section title}

even though all varieties are the same to LaTeX.  

For environments whose content does not conform to standard LaTeX  or
where graphical markup does not make sense all markup commands can be
removed by setting the PICTUREENV configuration variable (set by default to 
C<picture> environments; (see B<--config> option).

It is also possible to difference files which do not have a preamble. 
 In this case, the file is processed in the main document
mode, but the definitions of the markup commands are not inserted.

All markup commands inserted by I<latexdiff> begin with "C<\DIF>".  Added
blocks containing words, commands or comments which are in C<new.tex>
but not in C<old.tex> are marked by C<\DIFaddbegin> and C<\DIFaddend>.
Discarded blocks are marked by C<\DIFdelbegin> and C<\DIFdelend>.
Within added blocks all text is highlighted with C<\DIFadd> like this:
C<\DIFadd{Added text block}>
Selected `safe' commands can be contained in these text blocks as well
(use options to show and change the list of safe commands, see below).
All other commands as well as braces "{" and "}" are never put within
the scope of C<\DIFadd>.  Added comments are marked by prepending
"S<C<%DIF E<gt> >>".

Within deleted blocks text is highlighted with C<\DIFdel>.  Deleted
comments are marked by prepending "S<C<%DIF E<lt> >>".  Non-safe command
and curly braces within deleted blocks are commented out with 
"S<C<%DIFDELCMD E<lt> >>".



=head1 OPTIONS

=head2 Preamble

The following options determine the visual markup style by adding the appropriate
command definitions to the preamble. See the end of this section for a description of 
available styles.

=over 4

=item B<--type=markupstyle> or
B<-t markupstyle>

Add code to preamble for selected markup style. This option defines
C<\DIFadd> and C<\DIFdel> commands.
Available styles: 

C<UNDERLINE CTRADITIONAL TRADITIONAL CFONT INVISIBLE 
CHANGEBAR CCHANGEBAR CULINECHBAR CFONTCBHBAR>

[ Default: C<UNDERLINE> ]

=item B<--subtype=markstyle> or
B<-s markstyle> 

Add code to preamble for selected style for bracketing
commands (e.g. to mark changes in  margin). This option defines
C<\DIFaddbegin>, C<\DIFaddend>, C<\DIFdelbegin> and C<\DIFdelend> commands.
Available styles: C<SAFE MARGINAL DVIPSCOL>

[ Default: C<SAFE> ]

=item B<--floattype=markstyle> or
B<-f markstyle>

Add code to preamble for selected style which 
replace standard marking and markup commands within floats
(e.g., marginal remarks cause an error within floats
so marginal marking can be disabled thus). This option defines all 
C<\DIF...FL> commands.
Available styles: C<FLOATSAFE IDENTICAL>

[ Default: C<FLOATSAFE> ]

=item B<--encoding=enc> or 
B<-e enc>

Specify encoding of old.tex and new.tex. Typical encodings are
C<ascii>, C<utf8>, C<latin1>, C<latin9>.  A list of available encodings can be 
obtained by executing 

C<perl -MEncode -e 'print join ("\n",Encode->encodings( ":all" )) ;' >

[Default encoding is utf8 unless the first few lines of the preamble contain
an invocation C<\usepackage[..]{inputenc}> in which case the 
encoding chosen by this command is asssumed. Note that ASCII (standard
latex) is a subset of utf8]

=item B<--preamble=file> or
B<-p file>

Insert file at end of preamble instead of generating
preamble.  The preamble must define the following commands
C<\DIFaddbegin, \DIFaddend, \DIFadd{..},
\DIFdelbegin,\DIFdelend,\DIFdel{..},>
and varieties for use within floats
C<\DIFaddbeginFL, \DIFaddendFL, \DIFaddFL{..},
\DIFdelbeginFL, \DIFdelendFL, \DIFdelFL{..}>
(If this option is set B<-t>, B<-s>, and B<-f> options
are ignored.)


=item B<--show-preamble>

Print generated or included preamble commands to stdout.

=back

=head2 Configuration

=over 4

=item B<--exclude-safecmd=exclude-file> or
B<-A exclude-file> or  B<--exclude-safecmd="cmd1,cmd2,...">

=item B<--replace-safecmd=replace-file>

=item B<--append-safecmd=append-file> or 
B<-a append-file> or B<--append-textcmd="cmd1,cmd2,...">

Exclude from, replace or append to the list of regular expressions (RegEx)
matching commands which are safe to use within the 
scope of a C<\DIFadd> or C<\DIFdel> command.  The file must contain
one Perl-RegEx per line (Comment lines beginning with # or % are
ignored).  Note that the RegEx needs to match the whole of 
the token, i.e., /^regex$/ is implied and that the initial
"\" of the command is not included. The B<--exclude-safecmd>
option can be combined with either of the other two. B<--exclude-safecmd>
and B<--append-safecmd> can also take a comma separated list as input. If a
comma for one of the regex is required, escape it thus "\,". In most cases it
will be necessary to protect the comma-separated list from the shell by putting
it in quotation marks.

=item B<--exclude-textcmd=exclude-file> or
B<-X exclude-file> or B<--exclude-safecmd="cmd1,cmd2,...">

=item B<--replace-textcmd=replace-file>

=item B<--append-textcmd=append-file> or 
B<-x append-file> or B<--append-textcmd="cmd1,cmd2,...">

Exclude from, replace or append to the list of regular expressions
matching commands whose last argument is text.  See
entry for B<--exclude-safecmd> directly above for further details.

=item B<--config var1=val1,var2=val2,...> or B<-c var1=val1,..>

=item B<-c configfile>

Set configuration variables.
Available variables (see below for further explanations): 
    
C<MINWORDSBLOCK> (integer)
                          
C<FLOATENV> (RegEx)

C<PICTUREENV> (RegEx)

=item B<--show-safecmd>

Print list of RegEx matching and excluding safe commands.

=item B<--show-textcmd>

Print list of RegEx matching and excluding commands with text argument.

=item B<--show-config>

Show values of configuration variables

NB For all --show commands, no C<old.tex> or C<new.tex> file needs to be specified, and no 
differencing takes place.

=back

=head2 Miscellaneous

=over 4

=item B<--verbose> or B<-V>

Output various status information to stderr during processing.
Default is to work silently.

=item B<--help> or
B<-h>

Show help text

=item B<--version>

Show version number

=back

=head2 Predefined styles 

=head2 Major types

The major type determine the markup of plain text and some selected latex commands outside floats by defining the markup commands C<\DIFadd{...}> and C<\DIFdel{...}> .

=over 10

=item C<UNDERLINE>

Added text is underlined and blue, discarded text is struck out and red
(Requires color and ulem packages).

=item C<CTRADITIONAL>

Added text is blue and set in sans-serif, and a red footnote is created for each discarded 
piece of text. (Requires color package)

=item C<TRADITIONAL>

Like C<CTRADITIONAL> but without the use of color.

=item C<CFONT>

Added text is blue and set in sans-serif, and discarded text is red and very small size.

=item C<CCHANGEBAR>

Added text is blue, and discarded text is red.  Additionally, the changed text is marked with a bar in the margin (Requires color and changebar packages).

=item C<CFONTCHBAR>

Like C<CFONT> but with additional changebars (Requires color and changebar packages).

=item C<CULINECHBAR>

Like C<UNDERLINE> but with additional changebars (Requires color, ulem and changebar packages).

=item C<CHANGEBAR>

No mark up of text, but mark margins with changebars (Requires changebar package).

=item C<INVISIBLE>

No visible markup (but generic markup commands will still be inserted.

=back

=head2 Subtypes

The subtype defines the commands that are inserted at the begin and end of added or discarded blocks, irrespectively of whether these blocks contain text or commands (Defined commands: C<\DIFaddbegin, \DIFaddend, \DIFdelbegin, \DIFdelend>) 

=over 10

=item C<SAFE>

No additional markup (Recommended choice)

=item C<MARGIN>

Mark beginning and end of changed blocks with symbols in the margin nearby (using
the standard C<\marginpar> command - note that this sometimes moves somewhat
from the intended position.

=item C<DVIPSCOL>

An alternative way of marking added passages in blue, and deleted ones in red. Note
that C<DVIPSCOL> only works with the dvips converter, e.g. not pdflatex.
(it is recommeneded to use instead the main types to effect colored markup,
although in some cases coloring with dvipscol can be more complete).

=back

=head2 Float Types

Some of the markup used in the main text might cause problems when used within 
floats (e.g. figures or tables).  For this reason alternative versions of all
markup commands are used within floats. The float type defines these alternative commands.

=over 10

=item C<FLOATSAFE>

Use identical markup for text as in the main body, but set all commands marking the begin and end of changed blocks to null-commands.  You have to choose this float type if your subtype is C<MARGIN> as C<\marginpar> does not work properly within floats.

=item C<IDENTICAL>

Make no difference between the main text and floats.

=back


=head2 Configuration Variables

=over 10

=item C<MINWORDSBLOCK>

Minimum number of tokens required to form an independent block. This value is
used in the algorithm to detect changes of complete blocks by merging identical text parts of less than C<MINWORDSBLOCK> to the preceding added and discarded parts.

[ Default: 3 ]

=item C<FLOATENV>

Environments whose name matches the regular expression in C<FLOATENV> are 
considered floats.  Within these environments, the I<latexdiff> markup commands
are replaced by their FL variaties.

[ Default: S<C<(figure|table|plate)[\w\d*@]*> >]

=item C<PICTUREENV>

Within environments whose name matches the regular expression in C<PICTUREENV>
all latexdiff markup is removed (in pathologic cases this might lead to
 inconsistent markup but this condition should be rare).

[ Default: S<C<picture[\w\d*@]*> >]

=back

=head1 BUGS

UTF-8 support requires a relatively new version of perl (5.8.0 is sufficient 
but 5.6.2 up would work OK, too.

The current version is a beta version which has not yet been
extensively tested, but worked fine locally.  Please send bug reports
to I<tilmann@esc.cam.ac.uk>.  Include the serial number of I<latexdiff>
(from comments at the top of the source or use B<--version>).  If you come across latex
files that are error-free and conform to the specifications set out
above, and whose differencing still does not result in error-free
latex, please send me those files, ideally edited to only contain the
offending passage as long as that still reproduces the problem. 

=head1 SEE ALSO

L<latexrevise>

=head1 PORTABILITY

I<latexdiff> does not make use of external commands and thus should run
on any platform  supporting Perl 5.6 or higher.  If files with encodings 
other than ASCII or UTF-8 are processed, Perl 5.8 or higher is required.

The standard version of I<latexdiff> requires installation of the Perl package
C<Algorithm::Diff> (available from I<www.cpan.org> - 
I<http://search.cpan.org/~nedkonz/Algorithm-Diff-1.15>) but a stand-alone
version, I<latexdiff-so>, which has this package inlined, is available, too.

=head1 AUTHOR

Copyright (C) 2004 Frederik Tilmann

This program is free software; you can redistribute it and/or modify
it under the terms of the GNU General Public License Version 2

=cut


__END__
%%BEGIN SAFE COMMANDS
% Regex matching commands which can safely be in the
% argument of a \DIFadd or \DIFdel command (leave out the \)
arabic
dashbox
fbox
framebox
hspace
math.*
makebox
mbox
pageref
ref
symbol
raisebox
rule
text.*
shortstack
usebox
%%END SAFE COMMANDS

%%BEGIN TEXT COMMANDS
% Regex matching commands with a text argument (leave out the \)
addcontents.*
caption
cc
closing
chapter
dashbox
encl
fbox
framebox
footnote
footnotetext
framebox
part
(sub){0,2}section\*?
(sub)?paragraph\*?
makebox
mbox
opening
parbox
raisebox
savebox
sbox
shortstack
signature
value
underline
%%END TEXT COMMANDS 

%% TYPES (Commands for highlighting changed blocks)

%DIF UNDERLINE PREAMBLE
\RequirePackage[normalem]{ulem}
\RequirePackage{color}
\providecommand{\DIFadd}[1]{{\color{blue}\uline{#1}}}
\providecommand{\DIFdel}[1]{{\color{red}\sout{#1}}}                     
%DIF END UNDERLINE PREAMBLE

%DIF CTRADITIONAL PREAMBLE
\RequirePackage{color}
\providecommand{\DIFadd}[1]{{\color{blue} \sf #1}}
\providecommand{\DIFdel}[1]{{\color{red} [..\footnote{removed: #1} ]}}
%DIF END CTRADITIONAL PREAMBLE

%DIF TRADITIONAL PREAMBLE
\providecommand{\DIFadd}[1]{{\sf #1}}
\providecommand{\DIFdel}[1]{{[..\footnote{removed: #1} ]}}
%DIF END TRADITIONAL PREAMBLE

%DIF CFONT PREAMBLE
\RequirePackage{color}
\providecommand{\DIFadd}[1]{{\color{blue} \sf #1}}
\providecommand{\DIFdel}[1]{{\red{red} \scriptscriptsize #1}}
%DIF END CFONT PREAMBLE

%DIF CCHANGEBAR PREAMBLE
\RequirePackage[dvips]{changebar}
\RequirePackage{color}
\providecommand{\DIFadd}[1]{\cbstart{\color{blue}#1}\cbend}
\providecommand{\DIFdel}[1]{\cbdelete{\color{red}#1}\cbdelete}
%DIF END CCHANGEBAR PREAMBLE

%DIF CFONTCHBAR PREAMBLE
\RequirePackage[dvips]{changebar}
\RequirePackage{color}
\providecommand{\DIFadd}[1]{\cbstart{\color{blue}\sf #1}\cbend}
\providecommand{\DIFdel}[1]{\cbdelete{\color{red}\scriptscriptsize #1}\cbdelete}
%DIF END CFONTCHBAR PREAMBLE

%DIF CULINECHBAR PREAMBLE
\RequirePackage[normalem]{ulem}
\RequirePackage[dvips]{changebar}
\RequirePackage{color}
\providecommand{\DIFadd}[1]{\cbstart{\color{blue}\uline{#1}}\cbend}
\providecommand{\DIFdel}[1]{\cbdelete{\color{red}\sout{#1}}\cbdelete}
%DIF END CCHANGEBAR PREAMBLE

%DIF CHANGEBAR PREAMBLE
\RequirePackage[dvips]{changebar}
\providecommand{\DIFadd}[1]{\cbstart{#1}\cbend}
\providecommand{\DIFdel}[1]{\cbdelete}
%DIF END CHANGEBAR PREAMBLE

%DIF INVISIBLE PREAMBLE
\providecommand{\DIFadd}[1]{#1}
\providecommand{\DIFdel}[1]{}
%DIF END INVISIBLE PREAMBLE


%% SUBTYPES (Markers for beginning and end of changed blocks)

%DIF SAFE PREAMBLE
\providecommand{\DIFaddbegin}{}
\providecommand{\DIFaddend}{}
\providecommand{\DIFdelbegin}{}
\providecommand{\DIFdelend}{}
%DIF END SAFE PREAMBLE

%DIF MARGIN PREAMBLE
\providecommand{\DIFaddbegin}{\protect\marginpar{a[}}
\providecommand{\DIFaddend}{\protect\marginpar{]}}
\providecommand{\DIFdelbegin}{\protect\marginpar{d[}}
\providecommand{\DIFdelend}{\protect\marginpar{]}}
%DIF END BRACKET PREAMBLE

%DIF DVIPSCOL PREAMBLE
%Note: only works with dvips converter
\RequirePackage{color}
\RequirePackage{dvipscol}
\providecommand{\DIFaddbegin}{\nogroupcolor{blue}}
\providecommand{\DIFaddend}{\nogroupcolor{black}}
\providecommand{\DIFdelbegin}{\nogroupcolor{red}}
\providecommand{\DIFdelend}{\nogroupcolor{black}}
%DIF END DVIPSCOL PREAMBLE


%% FLOAT TYPES 

%DIF FLOATSAFE PREAMBLE
\providecommand{\DIFaddFL}[1]{\DIFadd{#1}}
\providecommand{\DIFdelFL}[1]{\DIFdel{#1}}
\providecommand{\DIFaddbeginFL}{}
\providecommand{\DIFaddendFL}{}
\providecommand{\DIFdelbeginFL}{}
\providecommand{\DIFdelendFL}{}
%DIF END FLOATSAFE PREAMBLE

%DIF IDENTICAL PREAMBLE
\providecommand{\DIFaddFL}[1]{\DIFadd{#1}}
\providecommand{\DIFdelFL}[1]{\DIFdel{#1}}
\providecommand{\DIFaddbeginFL}{\DIFaddbegin}
\providecommand{\DIFaddendFL}{\DIFaddend}
\providecommand{\DIFdelbeginFL}{\DIFdelbegin}
\providecommand{\DIFdelendFL}{\DIFdelend}
%DIF END IDENTICAL PREAMBLE

